An Uncertainty-Aware Approach for Exploratory Microblog Retrieval

Although there has been a great deal of interest in analyzing customer opinions and breaking news in microblogs, progress has been hampered by the lack of an effective mechanism to discover and retrieve data of interest from microblogs. To address this problem, we have developed an uncertainty-aware visual analytics approach to retrieve salient posts, users, and hashtags. We extend an existing ranking technique to compute a multifaceted retrieval result: the mutual reinforcement rank of a graph node, the uncertainty of each rank, and the propagation of uncertainty among different graph nodes. To illustrate the three facets, we have also designed a composite visualization with three visual components: a graph visualization, an uncertainty glyph, and a flow map. The graph visualization with glyphs, the flow map, and the uncertainty analysis together enable analysts to effectively find the most uncertain results and interactively refine them. We have applied our approach to several Twitter datasets. Qualitative evaluation and two real-world case studies demonstrate the promise of our approach for retrieving high-quality microblog data.

==> data.tex <==
% !TEX root = EvoTree-KDD.tex

\section{Background: }\label{sec:data}



==> discussion.tex <==
\section{Discussion}

==> overview.tex <==
\begin{figure*}[ht]
  \centering

  \includegraphics[width=\linewidth]{fig/overview}
  \caption{System pipeline: (a) generate evolving topic trees (dotted lines represent matched topics between times); (b) generate evolving tree cuts (the star is the user-selected focus node); (c) reorganize the topics according to the Degree-of-Interest (DOI) values; (d) align topic nodes by their depths; (e) color and scale topic nodes by the DOI values; (f) extract matched documents for the matched topics; (g) generate the final visualization.}\looseness=-1
  \label{fig:overview}
  \vspace{-3mm}
\end{figure*}

\section{Problem Formulation}
Fig.~\ref{fig:overview} briefly illustrates our system pipeline.
The input is a set of documents with time stamps.
First, we extract a sequence of topic trees from the input documents by our evolutionary tree clustering technique, which aims to better organize the topics at different times, as well as match correlated topics between adjacent topic trees.
Second, we transform tree clustering results into a set of salient topics that can well represent the large clustering results and be effectively visualized.
A user selects one or more topics of interest as the focus node(s).
Based on the focus node(s), the tree cut algorithm extracts a set of representative topics for each tree.
The algorithm also makes the representative topic sets at different times coherent with each other.
However, the cut algorithm may still extract too many topics that cannot be clearly displayed on the limited display area.
To tackle this, a mean-shift clustering algorithm~\cite{comaniciu2002mean} is employed to further group the extracted topics.
Meanwhile, the matched documents within the matched topics are extracted based on the relationships between the topics selected by our tree cut algorithm.
Finally, the transformed results, including the topics nodes on each tree cut, matched topics and documents, are visualized for further exploration and analysis.

==> quantative.tex <==
\begin{figure*}[t]
	\centering
	%\subfigure[1 focus (\emph{A})]{\label{fig:NMI_A1}
%	\includegraphics[width=0.235\linewidth]{./fig/NMI_A1.pdf}
%	}
%	\subfigure[3 foci (\emph{A})]{\label{fig:NMI_A3}
%	\includegraphics[width=0.235\linewidth]{./fig/NMI_A3.pdf}
%	}
%	\subfigure[1 focus (\emph{B})]{\label{fig:NMI_B1}
%	\includegraphics[width=0.235\linewidth]{./fig/NMI_B1.pdf}
%	}
%	\subfigure[3 foci (\emph{B})]{\label{fig:NMI_B3}
%	\includegraphics[width=0.235\linewidth]{./fig/NMI_B3.pdf}
%	}
    \includegraphics[width=\linewidth]{fig/nmi.pdf}
\vspace{-7mm}
	\caption{Comparison of NMI smoothness. X-axis represents tree index and y-axis encodes NMI smoothness.}\label{fig:NMI}
%\vspace{-2mm}
\end{figure*}

\begin{figure*}[t]
	\centering
%	\subfigure[1 focus (\emph{A})]{\label{fig:NMI_2A}
%	\includegraphics[width=0.235\linewidth]{./fig/TreeDistance_A1.pdf}
%	}
%	\subfigure[3 foci (\emph{A})]{\label{fig:rf-over-time}
%	\includegraphics[width=0.235\linewidth]{./fig/TreeDistance_A3.pdf}
%	}
%	\subfigure[1 focus (\emph{B})]{\label{fig:NMI_2A}
%	\includegraphics[width=0.235\linewidth]{./fig/TreeDistance_B1.pdf}
%	}
%	\subfigure[3 foci (\emph{B})]{\label{fig:rf-over-time}
%	\includegraphics[width=0.235\linewidth]{./fig/TreeDistance_B3.pdf}
%    }
    \includegraphics[width=\linewidth]{fig/distance.pdf}
\vspace{-7mm}
	\caption{Comparison of tree distance smoothness. X-axis represents tree index and y-axis encodes tree distance smoothness.}\label{fig:distance}
\vspace{-3mm}
\end{figure*}

\begin{table*}[b]

\vspace{-5mm}
    \caption{
%    \small
    Evaluation of the overall likelihood and smoothness.}
    $f_r(\cdot)=\frac{m_o-m_b}{m_b}*100\%$, where $m_b$ and $m_o$ are the metric values of the baseline method and our method.
    \label{table:average}
    \vspace{1mm}
    \centering \scalebox{0.8}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    &\multicolumn{3}{|c|}{$f_r(Likelihood)$(\%)} & \multicolumn{3}{|c|}{$f_r(\bm{S_{NMI}})$(\%)} & \multicolumn{3}{|c|}{$f_r(\bm{S_{dist}})$}& \multicolumn{3}{|c|}{$f_r(\bm{S_{map}})$(\%)}\\
    \hline
    & 1 focus & 2 foci & 3 foci& 1 focus & 2 foci& 3 foci& 1 focus& 2 foci & 3 foci& 1 focus& 2 foci & 3 foci\\
    \hline
   \emph{Dataset A} & 0.5137 & 0.1695 & 0.0991 & 13.1642 & 15.0561 & 16.1501 & -22.7957 & -27.3868 & -27.8560 & -29.5690 & -44.5076 & -40.4065\\
    \emph{Dataset B} & 0.4966 & 0.1793 & 0.0473 & 11.7578 & 12.4564 & 15.0249 & -9.4234 & -8.8731 & -15.8001 & -38.4656 & -38.2794 & -24.5879\\
    \emph{Dataset C} & 1.1031 & 0.5937 & 0.4655 & 7.7866 & 10.5127 & 10.1438 & -22.6327 & -24.4004 & -20.6693 & -48.1296 & -31.9426 & -20.6921\\
        \hline
    \end{tabular}
    }
  %  \vspace{-5mm}
\end{table*}

\begin{figure*}[t]
	\centering
	\subfigure[Dataset \emph{A}]{\label{fig:likelihood_A}
	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_A.pdf}
	}
	\subfigure[Dataset \emph{B}]{\label{fig:Likelihood_B}
\vspace{-2mm}
	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_B.pdf}
	}
    \subfigure[Dataset \emph{C}]{\label{fig:Likelihood_C}
\vspace{-2mm}
	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_C.pdf}
	}
%\hspace{1mm}
   \hspace{-8mm}
   \subfigure[Legend]{\label{fig:legend}

\vspace{-2mm}
	\includegraphics[width=0.2\linewidth]{./fig/Likelihood_legend.pdf}
	}
\vspace{-4mm}
	\caption{
%\small
Comparison of likelihood.}\label{fig:likelihood}
%\vspace{-2mm}
\end{figure*}

%\begin{figure*}[t]
%	\centering
%	\subfigure[Dataset \emph{A}]{\label{fig:tree_num}
%	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_A.pdf}
%	}
%	\subfigure[Dataset \emph{B}]{\label{fig:Likelihood_B}
%\vspace{-2mm}
%	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_B.pdf}
%	}
%    \subfigure[Dataset \emph{C}]{\label{fig:Likelihood_C}
%\vspace{-2mm}
%	\includegraphics[width=0.25\linewidth]{./fig/Likelihood_B.pdf}
%	}
%%\hspace{1mm}
%   \hspace{-8mm}
%   \subfigure[Legend]{\label{fig:legend}
%
%\vspace{-2mm}
%	\includegraphics[width=0.2\linewidth]{./fig/Likelihood_legend.pdf}
%	}
%\vspace{-4mm}
%	\caption{
%%\small
%Comparison of likelihood.}\label{fig:likelihood}
%\vspace{-2mm}
%\end{figure*}

%\begin{figure*}[b]
%\centerline
%{
%\includegraphics[width=0.235\linewidth]{./fig/Likelihood_A.pdf}
%\includegraphics[width=0.235\linewidth]{./fig/Likelihood_B.pdf}
%\includegraphics[width=0.235\linewidth]{./fig/Likelihood_B.pdf}
%\hspace{-6mm}
%\includegraphics[width=0.2\linewidth]{./fig/Likelihood_legend.pdf}
%}
%\centerline{
%Dataset \emph{A} \hspace{0.2\linewidth} Dataset \emph{B}  \hspace{0.2\linewidth} Dataset \emph{C} \hspace{0.2\linewidth} Dataset \emph{C}
%}
%\caption{Comparison of likelihood.}\label{fig:likelihood}
%\end{figure*}

\subsection{Quantitative Evaluation}
To assess the effectiveness of our evolutionary tree cut algorithm, we performed experiments on a number of different datasets.


\subsubsection{Criteria}
Fitness and smoothness were employed as two important criteria to evaluate the derived evolutionary tree cuts.
Likelihood was utilized to measure the fitness of a tree.
Three metrics were introduced to assess the smoothness between adjacent tree cuts.

\noindent\textbf{Tree mapping metric ($\bm{S_{map}}$}:
We derived the metric from the proposed global tree cut energy function, $\bm{S_{map}}=\mathbf{E}_1+\mathbf{E}_3$,
where $\mathbf{E}_1$ and $\mathbf{E}_3$ are defined in Eq.~(\ref{eq:energy}).
The smaller the $\bm{S_{map}}$ value, the smoother between two adjacent trees.
The following two criteria were then defined based on a metric of cluster quality and the tree structure.

\noindent\textbf{Normalized Mutual Information (NMI) ($\bm{S_{NMI}}$)}:
The NMI metric is defined as the mutual information between the cluster assignments and a pre-existing labeling.
Hungarian algorithm~\cite{Steiglitz1982} was employed to find the optimal match between the document sets of the two tree cuts.
This metric assess the similarity between adjacent tree cuts.
The larger the $\bm{S_{NMI}}$ value, the smoother between two adjacent trees.

\noindent\textbf{Tree distance ($\bm{S_{dist}}$)}:
We use this metric to measure the difference between tree cuts by aggregating the tree distance between two related cut nodes, $S_{Dist}=\frac{1}{\lambda}\log(p_{dist}(T^t|T^{t-1}))$.
Here $\log p_{dist}(T^t|T^{t-1})$ is defined by
\begin{equation}
\small
\log p_{dist}(T^t|T^{t-1}) \triangleq  -\lambda E_{T_r,T_s\in leaves(T^t) \atop r\ne s}(D_{T^t}(T_r,T_s)-D_{\tilde{T}^t}(T_r,T_s))^2,
\label{eq:distancemesaure}
\vspace{-1mm}
\end{equation}
where $D_T(T_r,T_s)$ is the tree distance between cut nodes $T_r$ and $T_s$, $\lambda$  is the weight balancing smoothness and tree likelihood.
The smaller the $\bm{S_{dist}}$ value, the smoother between two adjacent trees.


\subsubsection{Results}\label{sec:results}

We implemented a baseline system according to the seed tree cut generation method.
Specifically, a tree cut was derived for each time via Eq.~\ref{eq:seed} in the baseline method.
% and treated them as the baseline tree cuts.
To compare the fitness and smoothness of our methods to the baseline, we conducted experiments on the following three datasets.
\begin{compactitem}
%\item \textbf{an evolutionary hierarchial clustering method} that generates a sequence of coherent multi-branch topic trees;
\item \textbf{Paper dataset \emph{A}} that contains 3,860 research papers in data mining and visualization fields (2000 to 2010).
3,860 papers were organized yearly into 11 topic trees.
The tree depth, the total node number, and the first-level node number of the trees varied from 3 to 4, 32 to 82, and 10 to 33, respectively.
\item \textbf{News dataset \emph{B}} that includes 444,432 news articles related to ``Obama'' (Sep. 1, 2012 to Jan. 14, 2013).
The articles were organized into 18 topic trees by week.
The tree depths varied from 4 to 5, the total node numbers changed from 144 to 297, and the node number of the first level ranged from 18 to 79.\looseness=-1
\item \textbf{News dataset \emph{C}} that includes 1,023,104 news articles from 51 news sources such as York Times, Reuters, and BBC (Dec. 1, 2013 to Dec. 14, 2013).
The articles were organized into 14 topic trees by day.
The tree depths varied from 5 to 7, the total node numbers changed from 2,415 to 5,166, and the node
number of the first level ranged from 187 to 1,193.\looseness=-1
%\item \textbf{A news dataset \emph{C}} that contains 1,200,011 news articles.
\end{compactitem}

%\begin{figure*}[t]
%	\centering
%	\subfigure[Dataset \emph{A}]{\label{fig:NMI_1A}
%	\includegraphics[width=0.235\linewidth]{./fig/Likelihood_A.pdf}
%	}
%	\subfigure[Dataset \emph{B}]{\label{fig:NMI_2A}
%\vspace{-2mm}
%	\includegraphics[width=0.235\linewidth]{./fig/Likelihood_A.pdf}
%	}
%    \subfigure[Dataset \emph{C}]{\label{fig:NMI_2A}
%\vspace{-2mm}
%	\includegraphics[width=0.235\linewidth]{./fig/Likelihood_A.pdf}
%	}
%\vspace{-4mm}
%	\caption{Comparison of tree number.}\label{fig:likelihood}
%\vspace{-2mm}
%\end{figure*}


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{fig/obama}
  \vspace{-3mm}
  \caption{
%  \small
  (a) Overview of Obama data; (b) ``Tax'' and ''Debate'' related topics; (c) ``Iran'' and ''Debate'' related topics; (d) child topics in the ``Gun Control'' topic; (e) more child topics in the ``Gun Control'' topic.}
  \vspace{-3mm}
  \label{fig:obama}
\end{figure*}


To eliminate the bias caused by the focus node selection, we randomly selected the given number of focus nodes fifty times and ran the experiments fifty times.
The results were computed by averaging the 50 trials.

We compared the overall likelihood and smoothness with the baseline.
As shown in Table~\ref{table:average}, our method can generate a much smoother structure than the baseline while maintaining a larger likelihood.
Besides having very good performance under the metric of $\bm{S_{map}}$, our algorithm also achieved a comparable performance under the metrics of $\bm{S_{NMI}}$ and $\bm{S_{dist}}$.

Since the metric $\bm{S_{map}}$ is a global smoothness metric, so we further compared our method with the baseline between trees under the metrics $\bm{S_{NMI}}$ and $\bm{S_{dist}}$.
%First, we assessed the smoothness of our evolutionary tree cut algorithm based on the three different smoothness metrics.
As shown in Figs.~\ref{fig:NMI} and \ref{fig:distance}, the proposed evolutionary algorithm works pretty well under the commonly used metrics, NMI and tree distance.
The fitness of our algorithm at each tree was also evaluated.
As shown in Fig.~\ref{fig:likelihood}, the likelihood of our algorithm is as good as the baseline at each time in all the datasets.
This findings demonstrate that our algorithm can preserve the smoothness between trees without sacrificing the likelihood of each tree.
%Finally, we demonstrated that the performance of our algorithm consistently improved with the number of focus nodes.
%From Table~\ref{table:average}, we can see that the average likelihood difference decreases with the number of focus nodes, while the average smoothness difference increases with the number of focus nodes.
%This indicates that our algorithm works better when more focus nodes are selected.





